Stochastic Minimum Vertex Cover in General Graphs: a $3/2$-Approximation

Our main result is designing an algorithm that returns a vertex cover of $\mathcal{G}^\star$ with size at most $(3/2+\epsilon)$ times the expected size of the minimum vertex cover, using only $O(n/\epsilon p)$ non-adaptive queries. This improves over the best-known 2-approximation algorithm by Behnezhad, Blum, and Derakhshan [SODA'22], who also show that $\Omega(n/p)$ queries are necessary to achieve any constant approximation. Our guarantees also extend to instances where edge realizations are not fully independent. We complement this upper bound with a tight $3/2$-approximation lower bound for stochastic graphs whose edges realizations demonstrate mild correlations.

==> algfigure.tex <==
\begin{tikzpicture}
\definecolor{cadmium}{rgb}{0.0, 0.42, 0.24}

\draw[color=red, line width = 2mm] (0,0) -- (3, 0);
\draw[color=blue, line width = 2mm] (3,0) -- (12, 0);
\draw[color=red, line width = 2mm] (12,0) -- (15, 0);

\draw[color=red, line width = 1mm] (0, 0.3) -- (0,-0.3);
\draw[color=blue, line width = 1mm] (3, 0.3) -- (3,-0.3);
\draw[color=blue, line width = 1mm] (12, 0.3) -- (12,-0.3);
\draw[color=red, line width = 1mm] (15, 0.3) -- (15,-0.3);

\node at (0, -0.6) {\large $0$};
\node at (3, -0.6) {\large $1 - \tau - \epsilon$};
\node at (12, -0.6) {\large $\tau$};
\node at (15, -0.6) {\large $1$};
\end{tikzpicture}

==> intro-old.tex <==
\newcommand{\red}[1]{{\color{red}#1}}
\section{Introduction}

In the \emph{stochastic vertex cover} problem, we are given a base graph $G = (V, E)$ but  we do
not know which edges in $E$ actually exist. Rather each edge $e\in E$ is realized independently with a given existence probability $p_e \in (0,1]$, forming a subgraph $\mathcal{G}^\star$. Our goal is to find a minimum vertex cover of $\mathcal{G}^\star$.
While $\mathcal{G}^\star$ is unknown, one can verify its edge set by querying edges $e \in E$. 
Of interest, then, are algorithms that \emph{query a small subset of edges} and, based on the outcome of these queries, find a \emph{near-optimal vertex cover} of $\mathcal{G}^\star$.
How small should the set of queried edged %, i.e., \emph{the query-complexity} of the algorithm, 
be?
The gold standard in these problems is to non-adaptively issue a number of queries that is linear in  the number of vertices and polynomial in inverse probability $p = \min_{e\in E} p_e$. 


Algorithms for stochastic graphs have been studied primarily in regimes  where computationally-efficient algorithms were known for their non-stochastic counterparts, e.g., $(1-\epsilon)$-approximate maximum matchings~\cite{?}, minimum spanning trees~\cite{?}, $(1+\epsilon)$-approximate shortest paths~\cite{?}, and $2$-approximate minimum vertex cover~\cite{?}. 
This emphasis on efficiently solvable regimes is not accidental. 
By and large, structurally-simple properties that had long played a key role in understanding and designing computationally efficient algorithms have been used to guide an algorithm in its choice of queries.
These include the Tutte-Berge witness sets~\cite{AKL16}, short augmenting paths~\cite{blumetal}, and local computation~\cite{stoc20} in the stochastic matching problem and \red{.....} in a $2$-approximation for the stochastic minimum vertex problem. In these cases, a few queries of the random subgraph is sufficient to find, verify, or leverage these structurally-simple properties in algorithm design for the stochastic variant of the problem. 



For vertex cover beyond a $2$-approximation, and other computationally hard regimes,
hardness of computation~\cite{mvchard} has also been a barrier towards solving the stochastic variants of the problems. 
This is in part caused by lack of understanding regarding structural properties that impact the solution quality and can be learned from a small number of queries, even if they may not aid efficient computation.
To disentangle these computational and statistical challenges, we ask whether additional computational power can help break the $2$-approximation barrier in the stochastic minimum vertex cover.



\begin{question}
Can we achieve a better than $2$-approximation for the stochastic minimum vertex cover problem, using computationally inefficient algorithms? Can we do so efficiently, given access to an oracle for computing the minimum vertex cover of any graph?
\end{question}

Our paper answers both of these questions positively. At a high level, we introduce an algorithm that returns a  vertex cover of $\mathcal{G}^\star$ with probability $1$ whose sizes is at most $\frac{3}{2}$ times the expected minimum vertex cover of $\mathcal{G}^\star$. Moreover, our algorithm can be efficiently implemented using a polynomial number of queries to a minimum vertex cover oracle.

\begin{theorem}[Upper-bound] \label{thm:upper-mvc}
For any $\epsilon\in (0,0.1)$, there is an algorithm (namely Algorithm~\ref{}) that returns a $\left( \frac{3}{2}+\epsilon \right)$-approximate solution for the stochastic minimum vertex cover problem using $O\left(\frac{n}{\epsilon p}\right)$ queries. Moreover, this algorithm runs in time \red{....} given access an oracle for computing minimum vertex cover.
\end{theorem}

Interestingly, the approximation guarantees of Theorem~\ref{thm:upper-mvc} continue to hold even if edges of $\mathcal{G}^\star$ are correlated.
This allows us to handle \emph{mild correlations} in the realization of $\mathcal{G}^\star$. That is, even if  $O(n)$ edges are allowed to be realized in a correlated way, we can still achieve  a $\left( \frac{3}{2}+\epsilon \right)$-approximate solution using only  $O\left(\frac{n}{\epsilon p}\right)$ queries. 
Our next result shows that for such mildly correlated processes, a $\frac{3}{2}$-approximation is the best on can hope to get when using  $O\left(\frac{n}{\epsilon p}\right)$ queries. 


\begin{theorem}[Informal Lower Bound] \label{thm:lower-mvc}
There is a stochastic process for generating $\mathcal{G}^\star$ with $O(n)$ correlated edges\footnote{For a formal definition of a stochastic process with $O(n)$ correlated edges, see Definition~\ref{def:}}, such that any algorithm that returns a vertex cover of $\mathcal{G}^\star$ using only $O(n/\epsilon p)$ queries, must have an approximation ratio of at least $\frac32 - \epsilon$ with probability $1 - o(1)$.
\end{theorem}

Theorems~\ref{thm:upper-mvc} and \ref{thm:lower-mvc} together demonstrate that our results are tight, as long as there is even a small degree of correlations between the edges of $\cal{G}^\star$. This shows that to further go beyond the $3/2$-approximation one must fully leverage independence across all edges. We hope that this tight characterization of what is achievable for mildly correlated graphs may guide the design of new approaches that fully leverage independence to achieve a $(1+\epsilon)$-approximate minimum vertex cover.
Indeed, a similar characterization of what is achievable for correlated realization in the stochastic matching problem by~\cite{?} later inspired \cite{?} to enact a local model of computation to fully benefit from independence and give $(1-\epsilon)$-approximate matching. 

 


\begin{itemize}
    \item Our algorithm can be perceived as a specification algorithm since we only need to communicate $O(n)$ bits of information. This is unlike the previous work where after querying a subset of edges, they had to find an MVC of $O(m)$ edges.

\end{itemize}




\paragraph{Technical Overview/Algorithm design principal novelty ...y} The technical overview that we give two different prinipals for algorithm design for 2 approx. Partition to P and V minus P. Taking MVC of H plus P.

1. Chooses P using an outcome of MVC
2. Choosing P based on probability of MVC. 
They perform differently based on the distribution of Cv. To improve over the two approximation, we combine them in a smart way.
Smart way: acting differently




\section{alternative}
* General design and usage of cvs and ces. A note on their computation. A note on 2 approx versus better than 1 approx.

* General approach and template for alg: Commit to a set and query the rest. This is guaranteed to be an MVC. 
The queries graph has to then be guaranteed to have few edges.
Why this is obviously an MVC of the realization.
Where the algorithms defer is what set is committed to. 



We start with two algorithms both 2-approx. What is special about these two algs is that the
(can we say the sets these two algs commit to are different). Each performs better when cvs are larger or smaller.
We say how combining insights from these lead to a 1.5 approx.



\section{Preliminaries}
 \SetKwFunction{MVC}{MVC}
\begin{itemize}
\item Input of our problem is a base graph $G=(V, E)$ and a probability $p_e$ for any edge $e\in E$. 
\item We define $\mathcal{G}^*$ to be the actual realization of $G$ which contains each edge of $G$ independently with 	probability $p_e$.
\item Let $\text{MVC}$ be an algorithm that given any realization of $G$ return a minimum vertex cover. For any edge $e\in E$ we define $$c_e=\Pr[e \text{ has at least one end-point in MVC}(G_r)]$$ and for any vertex $v\in V$, we define $$c_v=\Pr[e \text{ is in MVC}(G_r)]$$ The probability here is taken over the randomization of the algorithm and realization of $G_r$.
\item
Mention $p = \min_{e\in E} p_e.$
\item $\opt=\text{MVC}(\mathcal{G}^\star)$.
\end{itemize}

==> related.tex <==
%\section{Further Related Work}


% %Aaron Bernstein
% %Sepehr Sepehr
% % Ole Svensson: Beating Greedy for Stochastic Bipartite Matching

% % https://arxiv.org/abs/1302.5913
% % https://arxiv.org/abs/1008.5356

% On stochastic submdular cover problem, see the commented links:
% %https://math.mit.edu/~goemans/PAPERS/stoch_cover_latin.pdf
% %

% On the interpretation of these results as price of stochasticity.



==> toolHSML.tex <==
\section{Tool I: The Half-Stochastic Matching Lemma}\label{sec:HSML}

The Half-Stochastic Matching Lemma, constructively, gives a partitioning $(Q, S)$ of the edge-set $E$ of graph $G$. This partitioning is accompanied with a special near-maximum matching algorithm $\mc{M}$ that operates on the ``half-stochastic'' random subgraph $H$ of $G$ in which each edge of $Q$ is stochastic (i.e. realized with probability $p$) and each edge of $S$ appears with probability one.  

Although this lemma seems to be about matchings only, it actually plays an important role in the stochastic vertex cover algorithm for Theorem~\ref{thm:bipartitevc} in both the algorithm in deciding which edges to query, and the analysis of the approximation ratio achieved by this algorithm. 

\begin{highlighttechnical}
\begin{lemma}[Half-Stochastic Matching Lemma]\label{lem:vcpartition}
\parindent=15pt
	Let $G=(V, E)$ be a (possibly non-bipartite) graph and let $\epsilon \in [0, 1]$ and $p \in [0, 1]$ be two given parameters. There is a partitioning of $E$ into  subsets $Q$ and $S$ such that:
\begin{enumerate}[itemsep=2pt, topsep=10pt,label={$(\roman*)$}]
		\item The maximum degree in $Q$ is $O(\frac{1}{\epsilon^{11} p^6})$.\label{vp-prop:degreeQ}
\end{enumerate}
Moreover, $Q$ and $S$ are such that there exists a randomized matching algorithm $\mc{M}$, where by letting $H := Q_p \cup S$ denote a random graph which includes all edges in $S$, but includes each edge of $Q$ independently with probability $p$, we get:
\begin{enumerate}[itemsep=2pt, topsep=10pt, label={$(\roman*)$}]
\setcounter{enumi}{1}
		\item $\E|\mc{M}(H)| \geq (1-2\epsilon) \cdot \E[\mu(H)]$. That is, the matching algorithm $\mc{M}$ should find an approximate maximum matching of $H$ in expectation. \label{vp-prop:expmatching}
		\item For any edge $e \in S$, $\Pr[e \in \mc{M}(H)] \leq \Stau$.\label{vp-prop:prsmallS}
	\end{enumerate}
	
	We note that the probabilistic statements above are with respect to both the inherent randomization in graph $H$, and also the randomization used in algorithm $\mc{M}$.
\end{lemma}
\end{highlighttechnical}

\newcommand{\threshD}[0]{\ensuremath{\epsilon^4 p}}
\newcommand{\SM}[1]{\ensuremath{\mc{M}_{#1}}}

We now turn to present the proof of Lemma~\ref{lem:vcpartition}. To do so, we have to output a triplet $(Q, S, \mc{M})$ where $Q$ and $S$ form a partitioning of $E$, and $\mc{M}$ is a matching algorithm. 

For some $k = O_{\epsilon, p}(1)$ which we specify later, we construct a list $(Q_0, S_0), (Q_1, S_1), \ldots, (Q_k, S_k)$ of partitionings. We will argue that if $k$ is large enough, there is one of the partitions, $(Q_i, S_i)$, which satisfies all the properties required by Lemma~\ref{lem:vcpartition}. This will be our partitioning $(Q, S)$.


\smparagraph{The construction.} The base partitioning is simply $Q_0 = \emptyset, S_0 = E$ and for each $i \geq 0$,  $(Q_{i+1}, S_{i+1})$ is constructed from the previous partitioning $(Q_i, S_i)$. To describe the construction, let us define for each partitioning $i$ a random graph $H_i$ which includes each edge of $Q_i$ independently with probability $p$, and includes every edge of $S_i$ with probability 1. We will also soon formalize a special randomized matching algorithm $\SM{i}$ that we run on graph $H_i$. Having $\SM{i}$, for each $i \geq 0$ we define
\begin{equation}\label{eq:defD}
	D_i := \{ e \in S_i \mid \Pr[e \in \SM{i}(H_i)] > \Stau \},
\end{equation}
and construct $(Q_{i+1}, S_{i+1})$ in the following way:
\begin{equation}\label{eq:constr-partitn}
	Q_{i+1} \gets Q_i \cup D_i \qquad \text{and} \qquad S_{i+1} \gets S_i \setminus D_i.
\end{equation}

Observe that in the construction above, each partitioning $(Q_{i+1}, S_{i+1})$ is obtained from the previous partitioning $(Q_{i}, S_{i})$ by ``moving'' the edges of $D_i$ (which are all by definition in $S_i$) from $S_i$ to partition $Q_i$. For this reason, we have
$$
	Q_0 \subset Q_1 \subset \ldots \subset Q_k \qquad \text{and} \qquad S_0 \supset S_1 \supset \ldots \supset S_k.
$$

Let us emphasize that graphs $H_0, H_1, \ldots, H_k$ have \textbf{different} distributions. Intuitively, since $Q_i$ grows as $i$ increases, and graph $H_i$ includes only $p$ fraction of the edges in $Q_i$ but all the edges in $S_i$, random graph $H_i$ tends to get smaller and smaller by increasing $i$. In fact it would be useful to consider a coupling $(H_0, H_1, \ldots, H_k)$ as follows: On each edge $e$ we draw an independent $p$-Bernouli random variable $X_e$ and use this to define $H_i$ for all $i$ as:
\begin{equation}\label{eq:coupling}
	H_i = \{e \mid (e \in Q_i \text{ and } X_e = 1) \text{ or } (e \in S_i)\}.
\end{equation}
This coupling is useful because in each outcome of the joint distribution $(H_0, \ldots, H_k)$, each graph $H_i$ is a subgraph of the previous graph $H_{i-1}$.


Let us now finalize our construction by formalizing algorithm $\SM{i}$.

\smparagraph{The Matching $\SM{i}$:} For any $i$ and any (possibly randomized) matching algorithm $\mc{M}'$, we define
\begin{equation}\label{eq:objective}
	\Phi_i(\mc{M}') := \sum_{e \in E} \left(\Pr_{\mc{M}', H_i}[e \in \mc{M}'(H_i)] - \epsilon \Pr_{\mc{M}', H_i}[e \in \mc{M}'(H_i)]^2\right),
\end{equation}
where let us emphasize that the probabilities are taken over both the possible randomization in algorithm $\mc{M}'$, and the randomization in graph $H_i$ (regarding the realization of edges belonging to $Q_i$). Having this definition, we now simply let $\SM{i}$ be the algorithm maximizing $\Phi_i$, i.e.:
$$
	\SM{i} := \argmax_{\mc{M}'} \Phi_i(\mc{M}'),
$$
and we use $\Phi_i := \Phi_i(\SM{i})$ to simply denote the optimal objective value obtained by this algorithm.

Let us, for now, not concern ourselves with how the objective function (\ref{eq:objective}) can be maximized in polynomial time and assume that this algorithm $\SM{i}$ is simply given. We will later address this issue and obtain a polynomial-time algorithm once it becomes clear how we use $\SM{i}$.

\smparagraph{The intuition behind objective $(\ref{eq:objective})$.} To see the intuition behind why we define the objective function (\ref{eq:objective}) this way, first note by linearity of expectation that
\begin{equation}\label{eq:sn123908}
	\Phi_i = \E|\SM{i}(H_i)| - \epsilon \sum_{e \in E} \Pr[e \in \SM{i}(H_i)]^2.
\end{equation}
The intuition behind the first term is clear: We want the expected size of the matching to be large;  Observation~\ref{obs:matchingSMlarge} below formalizes this by showing that the matching algorithm $\SM{i}$ maximizing $\Phi_i$ must be a $(1-\epsilon)$-approximate matching. The second term, on the other hand, ensures that the marginal probabilities of edges appearing in the matching tend to be small. This is useful for Property~\ref{vp-prop:prsmallS} of Lemma~\ref{lem:vcpartition} which requires small marginals for all edges in $S$.

\begin{observation}\label{obs:EM>Phi}
	For any $i$, $\E|\SM{i}(H_i)| \geq \Phi_i$.
\end{observation}
\begin{proof}
	By Equation (\ref{eq:sn123908}), $\E|\SM{i}(H_i)| = \Phi_i + \epsilon \sum_{e \in E} \Pr[e \in \SM{i}(H_i)]^2 \geq \Phi_i$.
\end{proof}

\begin{observation}\label{obs:matchingSMlarge}
	$\E|\SM{i}(H_i)| \geq (1-\epsilon) \cdot \E[\mu(H_i)]$.
\end{observation}
\begin{proof}
	Consider a deterministic algorithm $\mc{M}'$ that picks an arbitrary maximum matching $M$ of its random input $H_i$. Since $\E|M| = \E[\mu(H_i)]$, we have
	$$
	\Phi_i(\mc{M}') = \E[\mu(H_i)] - \epsilon \sum_{e \in E} \Pr[e \in M]^2 \geq \E[\mu(H_i)] - \epsilon \sum_{e \in E} \Pr[e \in M] = (1-\epsilon) \cdot \E[\mu(H_i)].
	$$
	Since $\SM{i}$ maximizes $\Phi_i = \Phi_i(\SM{i})$, we get $\Phi_i \geq \Phi_i(\mc{M}') \geq (1-\epsilon) \cdot \E[\mu(H_i)]$. Combined with $\E|\SM{i}(H_i)| \geq \Phi_i$ due to Observation~\ref{obs:EM>Phi}, this implies $\E|\SM{i}(H_i)| \geq (1-\epsilon) \cdot \E[\mu(H_i)]$.
\end{proof}


We now turn to prove that one of the partitionings $(Q_i, S_i)$ must satisfy the properties required by Lemma~\ref{lem:vcpartition}. The next set of claims are used for this purpose.

\begin{claim}\label{cl:matchingsdecreasing}
	It holds that
	$$
		\mu(G) \geq \Phi_0 \geq \Phi_1 \geq \ldots \geq \Phi_k \geq (1-\epsilon) \cdot p \cdot \mu(G).
	$$
\end{claim}

\begin{claim}\label{cl:interval}
	There is an interval $I = \{s, \ldots, s+k'\}$ in $[k]$ with $|I| \geq \frac{1}{300} \epsilon^6 p^3 k$ such that 
	\begin{flalign*}
		|\Phi_i - \Phi_j| \leq 0.01 \epsilon^6 p^3 \mu(G) \qquad\qquad \text{for all $i < j$ in $I$.}
	\end{flalign*}
\end{claim}

\begin{claim}\label{cl:Dicontinuestocontribute}
	Let $I$ be as defined in Claim~\ref{cl:interval}. Either there is some $i \in I$ where $\E|D_i \cap \SM{i}(H_i)| < \epsilon p \mu(G)$, or otherwise for any $i, j \in I$ with $i < j$, it holds that
	$$
		\E|D_i \cap \SM{j}(H_j)| \geq 0.25 \epsilon^3 p^2 \cdot  \mu(G).
	$$
\end{claim}

Claims~\ref{cl:matchingsdecreasing} and \ref{cl:interval} are proved in Section~\ref{sec:proofs-uh123} and Claim~\ref{cl:Dicontinuestocontribute} is proved in Section~\ref{sec:proof-dgl1298371923}. Claim~\ref{cl:Dicontinuestocontribute} is, in particular, the key part of the proof. It is proved by showing that if the condition of Claim~\ref{cl:Dicontinuestocontribute} is not satisfied, then the randomized matching algorithm that with probability $0.5$ picks the output of $\SM{j}(H_j)$ and otherwise the output of $\SM{i}(H_i)$, should obtain a larger objective than $\Phi_i$ which we show is a contradiction. 

Having proved these claims, we now turn to prove Lemma~\ref{lem:vcpartition}. 

\begin{proof}[Proof of Lemma~\ref{lem:vcpartition}]
First, we set $k = 5 \cdot \frac{300}{\epsilon^9 p^5}$. Since for any $i$, each edge in $D_i$ has probability at least $\epsilon^2 p$ of being in matching $\SM{i}(H_i)$, and that the probabilities around each vertex sum up to at most one, there are at most $\sfrac{1}{\epsilon^2 p}$ edges connected to each vertex in $D_i$. This implies that for any $j \in [k]$, $Q_j$ has maximum degree at most $k \cdot \frac{1}{\epsilon^2 p} = O(\frac{1}{\epsilon^{11} p^6})$, satisfying Property~\ref{vp-prop:degreeQ}. Now we prove there exists some $(Q_i, S_i)$ satisfying Properties~\ref{vp-prop:expmatching} and \ref{vp-prop:prsmallS} as well.

Let $I$ be as provided by Claim~\ref{cl:interval}. There are two possible cases:

	\smparagraph{Case 1 ---} There is some $i \in I$ where $\E|D_i \cap \SM{i}(H_i)| < \epsilon p \mu(G)$\textbf{:} 
	
	\noindent In this case, we can let $Q \gets Q_i, S \gets S_i,$ which implies graph $H$ of Lemma~\ref{lem:vcpartition} has the same distribution as $H_i$. We now let matching algorithm $\mc{M}$, required by Lemma~\ref{lem:vcpartition}, to be the same as matching algorithm $\SM{i}$, except that we exclude the edges of $D_i$ from the matching. That is, we let $\mc{M}(H) = \SM{i}(H_i) \setminus D_i$.

	Since we exclude the edges in $D_i$ from the matching,  we get that for all edges $e \in S$, $\Pr[e \in \mc{M}(H)] \leq \Stau$ satisfying Property~\ref{vp-prop:prsmallS}. On the other hand, 
	\begin{flalign*}
		\E|\mc{M}(H)| &= \E[ |\SM{i}(H_i) \setminus  D_i| ] = \E|\SM{i}(H_i)| - \E|D_i \cap \SM{i}(H_i)|\\
		&> \E|\SM{i}(H_i)| - \epsilon p \mu(G) \tag{By the assumption of Case 1.}\\
		&\geq (1-\epsilon) \E[\mu(H_i)] - \epsilon p \mu(G) \tag{By Observation~\ref{obs:matchingSMlarge}.}\\
		&\geq (1-2\epsilon) \E[\mu(H_i)] \tag{Since $\E[\mu(H_i)] \geq p\mu(G)$.}\\
		&= (1-2\epsilon) \E[\mu(H)]. \tag{Since $H$ and $H_i$ have the same distribution.}
	\end{flalign*}
	This proves $\mc{M}$ is a $(1-2\epsilon)$-approximate matching algorithm, satisfying Property~\ref{vp-prop:expmatching}.
	
	
	\smparagraph{Case 2 ---} For all $i \in I$, $\E|D_i \cap \SM{i}(H_i)| \geq \epsilon p \mu(G)$\textbf{:}
	
	\noindent In this case, by Claim~\ref{cl:Dicontinuestocontribute}, we have $\E|D_i \cap \SM{j}(H_j)| \geq 0.25 \epsilon^3 p^2 \cdot  \mu(G)$ for all $i < j$ in $I$. Let us denote $I = \{a_1, a_2, \ldots, a_{\ell}\}$ where $a_1 < \ldots < a_{\ell}$. Letting $j = a_{\ell}$, we thus get
	$$
		\E|D_{a_i} \cap \SM{a_\ell}(H_{a_\ell})| \geq 0.25 \epsilon^3 p^2 \cdot  \mu(G) \qquad\text{for all $i \in \{1, \ldots, \ell - 1\}$}.
	$$
	On the other hand, observe from construction (\ref{eq:constr-partitn}) that sets $D_{a_1}, \ldots, D_{a_{\ell - 1}}$ are all pairwise disjoint. This implies
	\begin{equation}\label{eq:bheug123981273}
		\E|\SM{a_\ell}(H_{a_\ell})| \geq \sum_{i=1}^{\ell - 1} \E|D_{a_i} \cap \SM{a_\ell}(H_{a_\ell})| \geq (\ell - 1) \cdot 0.25\epsilon^3 p^2 \cdot \mu(G).
	\end{equation}
	Recall from Claim~\ref{cl:interval} that $\ell = |I| \geq \frac{1}{300} \epsilon^6 p^3 k$. Since we set  $k = 5 \cdot \frac{300}{\epsilon^9 p^5}$, we get $\ell \geq \frac{5}{\epsilon^3 p^2}$ which combined with (\ref{eq:bheug123981273}) implies $\E|\SM{a_\ell}(H_{a_\ell})| > \mu(G)$ which is a contradiction since $H_{a_\ell}$ is a subgraph of $G$ and cannot have a larger matching than $\mu(G)$. This contradiction implies that if we set $k$ large enough, this second case essentially does not happen. As a result, we always end up at Case 1, which we just showed how it proves Lemma~\ref{lem:vcpartition}.

The proof of Lemma~\ref{lem:vcpartition} is thus complete.
\end{proof}

Finally, we remark that our techniques also lead to a partitioning with the same guarantee as in  Lemma~\ref{lem:vcpartition} that can be found in polynomial time. We defer the details of this polynomial-time implementation to Appnedix~\ref{apx:polytime}.


\subsection{Proofs of Claims~\ref{cl:matchingsdecreasing} and \ref{cl:interval}}\label{sec:proofs-uh123}
\begin{proof}[Proof of Claim~\ref{cl:matchingsdecreasing}]
	As discussed, in the coupling of Eq~\ref{eq:coupling}, $H_i$ is always a subgraph of $H_{i-1}$. As a result, matching algorithm $\SM{i}$ is also applicable on graph $H_{i-1}$, implying that $\Phi_{i-1} \geq \Phi_i$ for all $i$.
	
	To see why $\mu(G) \geq \Phi_0$, note from Observation~\ref{obs:EM>Phi} that $\E|\SM{0}(H_0)| \geq \Phi_0$. On the other hand, no matter what matching algorithm we use for $\SM{0}$, we have $\E|\SM{0}(H_0)| \leq \mu(G)$ as the output must be a matching in $H_0$ and thus $G$. Combining the two bounds gives $\mu(G) \geq \Phi_0$.
	
	Finally, to see why $\Phi_k \geq (1-\epsilon) \cdot p\cdot \mu(G)$, fix a maximum matching $M$ of $G$ which has to have size $\mu(G)$. Every edge $e \in M$ either is in $Q_k$ or $S_k$; in either case, $e \in H_k$ with probability at least $p$. We thus have $\E[\mu(H_k)] \geq \E|M \cap H_k| \geq p |M| = p \cdot \mu(G)$. Now consider a choice for $\SM{k}$ which deterministically picks a maximum matching $M_k$ of $H_k$. This proves
	\begin{flalign*}
		\Phi_k &\geq \sum_{e \in E} \Pr[e \in M_k] - \epsilon \Pr[e \in M_k]^2 \geq \sum_{e \in E} \Pr[e \in M_k] - \epsilon \Pr[e \in M_k]\\
		&= (1-\epsilon) \sum_{e \in E} \Pr[e \in M_k] 
		\geq (1-\epsilon) \cdot \E|M_k|
		= (1-\epsilon) \cdot \E[\mu(H_k)] 
		\geq (1-\epsilon) \cdot p \cdot \mu(G),
	\end{flalign*}
	completing the proof.
\end{proof}

\begin{proof}[Proof of Claim~\ref{cl:interval}]
	Let us define $I_j$ for any $j \in \{1, \ldots, \lceil 100/\epsilon^6 p^3\rceil\}$ as follows
	$$
		I_j := \{ i : (1- 0.01 j \epsilon^6 p^3) \mu(G) < \Phi_i \leq (1- 0.01 (j-1) \epsilon^6 p^3) \mu(G) \}.
	$$
	Recall from Claim~\ref{cl:matchingsdecreasing} that 
	$
		\mu(G) = \Phi_0 \geq \Phi_1 \geq \ldots \geq \Phi_k \geq (1-\epsilon)p\mu(G).
	$ 
	Thus, $I_1, I_2, \ldots$ partition $[k]$ into consecutive intervals where for all elements $i, j$ in the same interval, $|\Phi_i - \Phi_j| \leq 0.01 \epsilon^6 p^3 \mu(G)$.
	
	Since there are only $\lceil 100/ \epsilon^6 p^3 \rceil$ intervals and $\sum_j |I_j| = k$ (as every $i \in [k]$ belongs to exactly one of the intervals) there is at least one interval $I$ with $|I| \geq \frac{k}{\lceil 100/ \epsilon^6  p^3 \rceil + 1} > \frac{1}{300} \cdot \epsilon^6 p^3 k$. This interval $I$ satisfies the required property of the claim by its definition, and has the desired size.
\end{proof}

\subsection{Proof of Claim~\ref{cl:Dicontinuestocontribute}}\label{sec:proof-dgl1298371923}

\begin{proof}[Proof of Claim~\ref{cl:Dicontinuestocontribute}]
	Suppose for the sake of contradiction that 
	\begin{equation}\label{eq:gfc12839}
		\E|D_i \cap \SM{i}(H_i)| \geq \epsilon p \mu(G) \qquad \qquad \text{for all $i \in I$},
	\end{equation}
	and that there are $i, j \in I$ such that $i < j$ and 
	\begin{equation}\label{eq:bue129387}
		\E|D_i \cap \SM{j}(H_j)| <  0.25 \epsilon^3 p^2 \cdot \mu(G).
	\end{equation}
	Consider a matching $\SM{i, j}(H_i)$ which with probability $1/2$ returns the output of $\SM{i}(H_i)$ and with probability $1/2$ returns the output of $\SM{j}(H_j)$. Since $i < j$, by the coupling (\ref{eq:coupling}), $H_j$ is a subgraph of $H_i$ and thus any matching in $H_j$ is a matching in $H_i$. As a result, $\SM{i, j}$ is a valid matching algorithm for graph $H_i$. We prove that under (\ref{eq:gfc12839}) and (\ref{eq:bue129387}), algorithm $\SM{i, j}$ should satisfy $\Phi_i(\SM{i, j}) > \Phi_i(\SM{i})$ which contradicts the assumption that $\SM{i}$ maximizes $\Phi_i(\SM{i})$. 
	
	From the definition of objective $\Phi_i(\SM{i, j})$ we have
	\begin{flalign*}
		\Phi_i(\SM{i, j}) &= \sum_{e \in E} \Pr[e \in \SM{i, j}(H_i)] - \epsilon \Pr[e \in \SM{i, j}(H_i)]^2\\
		&= \sum_{e \in E} \left(\frac{\Pr[e \in \SM{i}(H_i)]+\Pr[e \in \SM{j}(H_j)]}{2}\right) - \epsilon \left(\frac{\Pr[e \in \SM{i}(H_i)]+\Pr[e \in \SM{j}(H_j)]}{2}\right)^2.
	\end{flalign*}
	Let us for simplicity of notation use $p_i(e) := \Pr[e \in \SM{i}(H_i)]$ and $p_j(e) := \Pr[e \in \SM{j}(H_j)]$. The equality above therefore can be expressed as
	\begin{equation}\label{eq:ce219837}
		\Phi_i(\SM{i, j}) = \sum_{e \in E} \left(\frac{p_i(e) + p_j(e)}{2} \right) - \epsilon \left(\frac{p_i(e) + p_j(e)}{2}\right)^2.
	\end{equation}
	Basic mathematical calculations give that for any $e$,
	\begin{flalign}
		\nonumber \left(\frac{p_i(e) + p_j(e)}{2}\right)^2 &= \frac{p_i(e)^2 + p_j(e)^2 +2p_i(e)p_j(e)}{4}\\
		\nonumber &= \frac{p_i(e)^2}{2} + \frac{p_j(e)^2}{2} - \frac{p_i(e)^2}{4} - \frac{p_j(e)^2}{4} + \frac{2p_i(e)p_j(e)}{4}\\
		&= \frac{p_i(e)^2}{2} + \frac{p_j(e)^2}{2} - \left( \frac{p_i(e) - p_j(e)}{2} \right)^2.\label{eq:gc128937123}
	\end{flalign}
	Replacing (\ref{eq:gc128937123}) back into (\ref{eq:ce219837}) gives
	\begin{flalign*}
		\Phi_i(\SM{i, j}) &= \sum_{e \in E} \left(\frac{p_i(e) + p_j(e)}{2} \right) - \epsilon \left( \frac{p_i(e)^2}{2} + \frac{p_j(e)^2}{2} - \left( \frac{p_i(e) - p_j(e)}{2} \right)^2 \right) \\
		&= \sum_{e \in E} \left(\frac{p_i(e) - \epsilon p_i(e)^2}{2}  \right) + \left(\frac{p_j(e) - \epsilon p_j(e)^2}{2}  \right) + \epsilon \left( \frac{p_i(e) - p_j(e)}{2} \right)^2.
		\tag{By simply moving the terms in the previous line.}\\
		&= \frac{\Phi_i}{2} + \frac{\Phi_j}{2} + \epsilon \sum_{e \in E} \left( \frac{p_i(e) - p_j(e)}{2} \right)^2 \tag{See below.}\\
		&\geq \Phi_i - 0.01\epsilon^6 p^3 \mu(G) + \epsilon \sum_{e \in E} \left( \frac{p_i(e) - p_j(e)}{2} \right)^2 \tag{Since $|\Phi_i - \Phi_j| \leq 0.01 \epsilon^6 p^3 \mu(G)$ by Claim~\ref{cl:interval}.}
	\end{flalign*}
	The third equality above, simply comes from the definition (\ref{eq:objective}) for $\Phi_i$, which implies $\Phi_i = \sum_e \Pr[e \in \SM{i}(H_i)] - \epsilon \Pr[e \in \SM{i}(H_i)]^2 = \sum_e p_i(e) - \epsilon p_i(e)^2$, and from the same bound applied on $\Phi_j$.
	
	Now define subset $D'_i := \{ e \in D_i \mid p_j(e) < 0.5 \epsilon^2 p \}$ of $D_i$. Using this subset only instead of the set $E$ of edges in the inequality above gives
	\begin{flalign*}
		\Phi_i(\SM{i, j}) &\geq \Phi_i - 0.01\epsilon^6 p^3 \mu(G)  + \epsilon \sum_{e \in D'_i} \left( \frac{p_i(e) - p_j(e)}{2} \right)^2 \\
		&\geq \Phi_i - 0.01\epsilon^6 p^3\mu(G) + \epsilon \sum_{e \in D'_i} \left(\frac{\epsilon^2 p - 0.5 \epsilon^2 p}{2}\right)^2 \tag{Since for any $e \in D'_i$, $p_j(e) < 0.5\epsilon^2 p$ by definition of $D'_i$ and $p_i(e) \geq \epsilon^2 p$ by definition of $D_i$.}\\
		&= \Phi_i - 0.01\epsilon^6 p^3 \mu(G) + \epsilon \sum_{e \in D'_i} \frac{\epsilon^4 p^2}{16}\\
		&= \Phi_i - 0.01\epsilon^6 p^3 \mu(G)  + \frac{\epsilon^5 p^2}{16} |D'_i|.
	\end{flalign*}
	To obtain the claimed contradiction, we will  prove that 
	\begin{equation}\label{eq:cgy182379123}
		|D'_i| \geq 0.5 \epsilon p \mu(G),
	\end{equation}
	which combined by inequality above proves
	\begin{equation}\label{eq:htcr1823973}
		\Phi_i(\SM{i, j}) \geq \Phi_i - 0.01\epsilon^6 p^3 \mu(G) + \frac{\epsilon^6 p^3}{32} \mu(G) >  \Phi_i + 0.01 \epsilon^6 p^3 \mu(G),
	\end{equation}
	which contradicts $\Phi_i$ being the maximum objective achievable.
	
	To complete the proof, it thus only remains to prove (\ref{eq:cgy182379123}). We have
	$$
		\E|D_i \cap \SM{j}(H_j)| = \sum_{e \in D_i} p_j(e)  = \sum_{e \in D_i \setminus D'_i} p_j(e) + \sum_{e \in D'_i} p_j(e) \geq \sum_{e \in D_i \setminus D'_i} p_j(e) \geq (|D_i| - |D'_i|) 0.5 \epsilon^2 p.
	$$
	Also note that 
	$$
		\epsilon p \mu(G) \stackrel{(\ref{eq:gfc12839})}{\leq} \E|D_i \cap \SM{i}(H_i)| = \sum_{e \in D_i} p_i(e) \leq \sum_{e \in D_i} 1 = |D_i|.
	$$
	Combining the two bounds above gives
	$$
		\E|D_i \cap \SM{j}(H_j)| \geq (\epsilon p \mu(G) - |D'_i|) 0.5 \epsilon^2 p = 0.5 \epsilon^3 p^2 \mu(G) - 0.5 \epsilon^2 p|D'_i|,
	$$
	which combined with the bound $\E|D_i \cap \SM{j}(H_j)| < 0.25 \epsilon^3 p^2 \cdot \mu(G)$ of (\ref{eq:bue129387}) gives
	$$
		0.25\epsilon^3 p^2 \mu(G) > 0.5 \epsilon^3 p^2 \mu(G) - 0.5 \epsilon^2 p |D'_i|.
	$$
	By moving the terms, we get
	$$
		|D'_i| > \frac{0.25 \epsilon^3 p^2 \mu(G)}{0.5 \epsilon^2 p} = 0.5 \epsilon p \mu(G).
	$$
	This is the desired bound of inequality (\ref{eq:cgy182379123}), which as discussed above completes the proof.
\end{proof}

